DataSculpt: Crafting Data Landscapes for Long-Context LLMs through Multi-Objective Partitioning

In recent years, Large Language Models (LLMs) have demonstrated significant improvements across a variety of tasks, one of which is the long-context capability. The key to improving long-context performance lies in effective data organization and management strategies that integrate data from multiple domains and optimize the context window during training. Through extensive experimental analysis, we identified three key challenges in designing effective data management strategies that enable the model to achieve long-context capability without sacrificing performance in other tasks: (1) a shortage of long documents across multiple domains, (2) effective construction of context windows, and (3) efficient organization of large-scale datasets. To address these challenges, we introduce DataSculpt, a novel data management framework designed for long-context training. We first formulate the organization of training data as a multi-objective combinatorial optimization problem, focusing on attributes including relevance, homogeneity, integrity, and efficiency. Specifically, our approach utilizes a coarse-to-fine methodology to optimize training data organization both efficiently and effectively. We begin by clustering the data based on semantic similarity (coarse), followed by a multi-objective greedy search within each cluster to score and concatenate documents into various context windows (fine). Our comprehensive evaluations demonstrate that DataSculpt significantly enhances long-context training performance, resulting in improvements of 18.09% in retrieval augmentation, 21.23% in summarization, 21.27% in reading comprehension, and a 3.81% increase in code completion, while also maintaining overall model proficiency with a 4.88% improvement.

==> chapters/intro.tex <==
% 八股文模板：
% Intro里分几个段落分别介绍Challenge，最好配上1）实验 或者 2）图例 佐证
% 重点 highlight Challenge 而不是 solution，然后总结 contribution 也从这几个层面来说

% 立意：长文本与短文本协同训练 → 如何将短文本构造成成合适的长文本？
% \textbf{Thesis}: Collaborative Training of Long and Short Texts → How to Construct Short Texts into Suitable Long Texts?

% for VLDB, highlight data management

% comments from Xiaonan
% \XN{para1: Background and Application of Long context in LLM} 
% classification of long context training: pre-train, post-train

% Large Language Models (LLMs) have become a cornerstone in the field of Artificial Intelligence (AI)~\cite{brown2020language,achiam2023gpt,lewkowycz2022solving}, particularly in Natural Language Processing tasks. Their emergence has significantly transformed the landscape of AI research and application, leading to unprecedented success across a myriad of benchmarks and real-world applications~\cite{dwivedi2021artificial}.
% Large Language Models (LLMs) have become a cornerstone in Artificial Intelligence (AI)~\cite{brown2020language,achiam2023gpt,lewkowycz2022solving}, particularly for Natural Language Processing (NLP) tasks. 
% Managing long sequences efficiently in transformer-based language modeling is a pivotal area of research that has garnered substantial attention in recent years~\cite{vaswani2017attention}. 
% long context
% shrinked version

% LLM 总体概述 → long context LLMs 的意义 && 痛点
\blue{The first sentence should better connect the significance of LLM (Large Language Models) to databases and data management. The current version leans too much towards ML community.}
% Large Language Models (LLMs) have become a cornerstone in Artificial Intelligence (AI)~\cite{brown2020language,achiam2023gpt,lewkowycz2022solving}, particularly for Natural Language Processing (NLP) tasks, reshaping AI research and applications with unparalleled success across benchmarks and real-world scenarios~\cite{dwivedi2021artificial}.
Large Language Models (LLMs) are revolutionizing Database and Data Management by enhancing natural language querying~\cite{xx}, query optimization~\cite{xx}, and semantic search~\cite{xx}, improving data retrieval~\cite{xx} and reasoning across datasets, thus pushing the boundaries of intelligent data systems.
Long context sequence enables LLMs to perform tasks significantly beyond existing paradigm~\cite{fu2024data}, making it a pivotal area of research that has garnered substantial attention in recent years~\cite{vaswani2017attention}.
However, LLMs' efficacy in processing long context does not consistently meet the expected standards.
Furthermore, despite claims of its feasibility, simply extending the training context window of LLMs does not guarantee an improvement in the long context modeling capabilities~\cite{li2024can}.
Hence, there is a compelling call for innovative strategies and methods to effectively cultivate the long context capabilities of LLMs. 


% comments from Xiaonan
% \XN{Challenge of Long context in LLM}
% already claimed in the previous paragraph

% importance of data management
Data plays a fundamental role during the training phases of LLMs~\cite{miao2024demystifying,fernandez2023large,data_collection_vldb}. 
While the significance of model architectures is widely acknowledged, data-focused approaches hold substantial importance~\cite{wang2023data}. 
The strategic management of data, especially in constructing an appropriately tailored training dataset, is critical for synergizing model performance and streamlining training processes across both pretraining and supervised fine-tuning stages~\cite{wang2023data,data_management4ML_sigmod}. 
% 先前工作, 着手点：model && data (强调 data !)
% In previous research, there have been efforts made in enhancing LLMs' capabilities for long context processing.
% % modify model architecture
% Context extensions methods~\cite{tworkowski2024focused,roziere2023code,peng2023yarn} concentrate on improving the model structure to accommodate training with long contexts.
% % FoT~\cite{tworkowski2024focused}
% % CodeLlama (CL)~\cite{roziere2023code} approach
% % yarn~\cite{peng2023yarn}
% While the significance of model architectures is widely acknowledged, data-focused approaches hold substantial importance~\cite{wang2023data}.
% Data-centric efforts have been made to explore the enhancement of model capabilities for long context processing.
% There have been data managements efforts made in exploring the enhancement of model capabilities for long context processing. 
Efforts in data management have been directed towards exploring ways to enhance model capabilities for processing long contexts.
% ICP (ICLM)
ICLM~\cite{shi2023context} situates related documents within the same context, thereby exposing LLMs to extensive relevant contexts and supplying training indicators that transcend document boundaries. 
% SPLICE
Similarly, SPLICE~\cite{staniszewski2023structured} utilized retrieval methodologies such as BM25~\cite{robertson2009probabilistic} and Contriever-MSMARCO~\cite{izacard2021unsupervised} to execute structured packing within the training context, with a focus on code-related data.
% primary
% importance of selection && scheduling for long context data
% Hence, there is a compelling call for the selection and scheduling of training data intended for bolstering the long context capabilities of LLMs.
% However, this method of concatenation can lead to cross-document attention within a sequence, which is neither a desirable learning signal nor computationally efficient.(cite)
% 针对 ICP, SPLICE 的劣势
However, given that each document in the training corpus is accessed only once, the strategy employed in the previous approaches yields a notable quantity of isolated documents. As a result, during the later stages, this leads to the concatenation of unvisited documents with relatively low semantic correlation. 
% 过渡到 challenges
Simultaneously, considering the current state of extended context sequences used for training, it leads to three key challenges:

% 对于 token number 的描述图
\begin{figure*}[h]
    \centering
    \includesvg[width=\textwidth]{figures/domain_normalized_stacked_bar_chart_new.svg}
    \caption{Distribution of token counts for individual documents across different domains. Domains are arranged in descending order from top to bottom based on the proportion of documents with token numbers exceeding 64K. Documents within the domains of books and academic papers predominantly feature medium to long lengths (L $\ge$ 16K), in contrast to other fields, especially web-sourced data, where document lengths are almost exclusively below 4K.}
    \label{fig:domain_stacked_barchart}
\end{figure*}

% 移回 method
% \begin{figure*}[h]
%     \centering
%     \includesvg[width=\textwidth]{figures/illustration_v2.svg}
%     \caption{Illustration of DataSculpt. 
%     % In the data preprocessing phase, we first segment documents into chunks with $\leq$ context length $L$, and embed the truncated chunks into vectors. During the semantic clustering phase, we adapt the varient of ISODATA equipped with FAISS index to cluster the semantically related documents. Subsequently, we employ greedy semantic-driven largest-fit algorithm to construct suitable sequences for extended-context training.
%     In the data preprocessing stage, documents are initially divided into chunks with $\leq$ context length $L$, which are subsequently transformed into vector embeddings. During the semantic clustering phase, we implement a variant of the ISODATA algorithm, which is augmented with the FAISS vector searching library, to aggregate documents based on semantic similarity. Following this, a greedy semantic-driven largest-fit algorithm is utilized to arrange these clusters into sequences that are multi-objective optimally configured for extended-context training.}
%     \label{fig:illustration}
% \end{figure*}

% challenge
% version 1
% \textbf{C1. Insufficient long training corpora.}
% The challenge lies in the scarcity of extensive and diverse training datasets that encompass long-context sequences.
% Documents with long sequences are conspicuously scarce in the training corpus~\cite{devries2023long}. For instance, less than 5\% of documents within CommonCrawl exceed 2k tokens in length.
% If unaddressed, the limited long training corpora hinders LLMs' exposure to complex narratives, thereby compromising their proficiency in understanding and generating long-form content~\cite{devlin2018bert}. 

% version 2
% **Challenge: Balancing Domain Diversity in Extended-Context Training**
% \textbf{C1. Optimizing long-context data while preserving domain diversity.} 
% \textbf{C1. Insufficient Long Training Corpora with Balanced Domain Mixtures.} 
\textbf{C1. Insufficient Domain-Balanced Long Training Corpora.}
% \textbf{C1. Extended-context training with balanced domain mixture.}
The challenge lies in effectively incorporating a wide range of domains into extended-context LLM training. Achieving a balanced domain mixture is imperative, since each domain encompasses distinct knowledge. 
However, the distribution of text lengths varies substantially across various domains, as depicted in \Cref{fig:domain_stacked_barchart}. 
While some domains offer data lengths suitable for long-context training, other domains, particularly web-sourced data where less than 1\% of documents exceed 4K tokens, necessitate the concatenation of multiple documents to achieve adequate training contexts. 
This may lead to increased cross-attention among different documents within sequences, which is an undesirable learning signal. 
% Addressing this challenge is essential for compromising LLMs' proficiency in understanding and generating content across a broad spectrum of knowledge areas.

% Consequently, a compounded challenge emerges: developing strategies to not only source and compile extensive, varied training datasets that adequately represent long-context sequences but also to ensure a balanced domain mixture. Addressing this challenge is vital for advancing LLM capabilities in understanding and generating long-form content, taking into account the distinct characteristics and knowledge encapsulated within different domains.


\textbf{C2. Absence of Criteria for Long Context Construction.}
While existing work has demonstrated the positive impact of structured data on amplifying language models' long-context capabilities~\cite{levine2021inductive,chan2022data,devries2023long,devlin2018bert}, these efforts remain preliminary. 
Research dedicated to the organization and quality assessment of long-sequence training data for LLMs tends to focus on a narrow set of factors, lacking a systematic framework. 
Consequently, there is a discernible need for a detailed and cohesive framework that systematically organizes training data for applications requiring extensive context. 
% A gap remains in the provision of a detailed and cohesive framework for the methodical organization and structuring of training data tailored for long-context applications.
% They have yet to provide a comprehensive framework for the systematic organization of long-context training data, which is needed in counteracting the dearth of training corpora with long sequences.


% Enhancing Large Language Models (LLMs) to improve their capabilities with long text sequences during the post-training phase presents a significant challenge, primarily due to the difficulty in constructing high-quality long sequence data. 
% This challenge necessitates a strategy that allows for the joint training of LLMs using both short and long sequence data. 

% version 1
% 以下 challenge 侧重于 data management
\textbf{C3. Efficiency in Massive Data Management.} 
% Training LLMs is an inherently resource-intensive process, requiring the processing of vast amounts of textual data to learn complex language patterns~\cite{brown2020language}. In this scenario, the effectiveness with which massive datasets are managed and scheduled significantly influences the training duration, financial outlay, and environmental impact of developing such models. Consequently, identifying and implementing efficient data scheduling strategies is crucial for advancing LLM capabilities in a sustainable manner. 
% Training LLMs from scratch with extended contexts is extremely time-consuming and labor-intensive.
% version 2
% 表达 2 个观点：training long context LLM from scratch 代价开销太大，所以更多目光都关注于 post-train；对于海量预训练数据进行长窗口组织的开销也非常大
% \textbf{C3. Efficiency in long context training.} 
Training LLMs with extended contexts from scratch is notably resource-intensive, requiring considerable time and labor investments~\cite{chen2024long}, which has redirected emphasis towards post-training optimizations as a more feasible strategy~\cite{ibrahim2024simple}. 
% This considerable demand on resources has shifted the focus towards post-training optimizations as a more viable approach. 
Furthermore, organizing extensive pretraining datasets into long-context sequences poses substantial logistical hurdles~\cite{big_data_management_vldb}, further compounding the complexity of developing LLMs efficiently. 
Consequently, devising and implementing strategies for efficient data scheduling and management is essential to enhance the capabilities of LLMs in a sustainable and cost-effective manner~\cite{data_production4ML_sigmod}, balancing the need for extensive context processing with the practical limitations of resource availability. 

% The efficiency of massive data scheduling in this context directly impacts the speed, cost, and environmental footprint of model training. 
% % 待修改
% The training of LLMs is fundamentally a resource-intensive endeavor, necessitating the analysis of extensive textual datasets to capture intricate language structures~\cite{brown2020language}. In this scenario, the effectiveness with which massive datasets are managed and scheduled significantly influences the training duration, financial outlay, and environmental impact of developing such models. Consequently, the identification and execution of optimized data scheduling methodologies are imperative for enhancing the capabilities of LLMs in an ecologically and economically sustainable fashion. 


% 本工作做了什么
% 在本工作中，为了解决以上问题，我们提出了DataSculpt，将长窗口训练数据的组织转化为一个多目标优化问题并进行分阶段贪婪求解的数据组织框架，如图1所示。在长窗口训练数据的组织过程中同时考虑Relevance，Homogeneity， Integrity和计算效率开销等多个目标，并进行分阶段贪婪求解从而达到训练数据有效组织的目的。我们对7B大小的模型分别进行了16K, 32K, 64K窗口大小的15B tokens的post-train，并 evaluate these models on tasks covering general understanding, summarization, reading comprehension, retrieval augmentation and code completion等方面。实验结果表明 DataSculpt 数据组织框架可以在少量训练tokens的情况下有效提升模型在post-train阶段的长窗口训练效果。
% tokens： 17,920,000,000
To address these issues, we introduce \textit{DataSculpt}, a novel framework designed to reconfigure the organization of extended-context training data into a multi-objective combinatorial optimization problem, as illustrated in \Cref{fig:illustration}. 
% This problem is subsequently tackled using a phased greedy algorithm, as depicted in \Cref{fig:illustration}. 
DataSculpt meticulously balances several critical objectives throughout the data organization process, including relevance, homogeneity, integrity, as well as computational efficiency, adopting a coarse-to-fine methodology to optimize the architecture of training data. 
We conducted post-training with 15 billion tokens on a 7B model across varying sequence lengths of 16K, 32K, and 64K,
% , and evaluated these models on tasks encompassing general understanding, summarization, reading comprehension, retrieval augmentation, and code completion. 
and experimental results demonstrate that DataSculpt improves performance in an array of tasks, most significantly in general understanding (+4.88\%), retrieval augmentation (+18.09\%), summarization (+21.23\%), reading comprehension (+21.27\%) and code completion (+3.81\%). 
The finding reveals that DataSculpt can markedly synergize the model’s performance in long-context utilization during the post-train phase, even with a constrained number of training tokens.
% Experimental results demonstrate that DataSculpt can markedly boost the model’s performance in long-context training during the post-train phase, even with a constrained number of training tokens.

% contribution
Our contributions can be summarized as follows:
\begin{itemize}
    % \item We highlight the issue of assembling an appropriate long-context training corpus with balanced domain mixtures, a task pivotal for improving LLMs' capabilities in processing long text sequences.
    \item We highlight the challenge of compiling an appropriate long-context training corpus with a balanced domain mixture, crucial for enhancing the capabilities of LLMs in processing extensive text sequences.
    % \item We propose DataSculpt, a highly efficient framework for constructing suitable long context training data, which applies multi-objective allocation to extended sequence construction.
    \item To create suitable long context training data, we propose an efficient framework DataSculpt, which employs a multi-objective partition allocation strategy for the construction of extended context sequences. 
    \item Through quantitative analysis and t-SNE visualization of clustering outcomes at the intermediary stage of DataSculpt, we validate DataSculpt's robustness for multi-objective data concatenation within extended sequences.
    % \item We have engaged in continual pretraining with different context lengths on a 7B model using DataSculpt, and conducted evaluation on 17 tasks to demonstrate the efficacy of our proposed method.
    \item We engaged in continual pretraining using DataSculpt with various context lengths on a 7B model, and subsequently assessed its performance across 17 distinct tasks, illuminating the profound impact of our proposed method.
    % \item Study: Analysis of experimental results?
\end{itemize}

% comments from Xiaonan
% \XN{Paper Orgnization}

==> chapters/related_work.tex <==
\subsection{Training Long-Context Language Models}

% long context training 的意义
Training Large Language Models (LLMs) with expanded context windows facilitates the execution of tasks that surpass the capabilities defined by the existing paradigm, such as multi-document question answering~\cite{caciularu2023peek}, long document summarization~\cite{bai2023longbench}, and enhanced retrieval functionalities~\cite{liu2024lost}.
% 但是训练长窗口模型开销很大
Nevertheless, the endeavor of training LLMs with extended contexts is notably time-consuming and labor-intensive. 
% data-centric 方面：long context 数据稀缺
Furthermore, documents with long sequences are conspicuously scarce in the training corpus~\cite{devries2023long}. For instance, less than 5\% of documents within CommonCrawl exceed 2k tokens in length~\cite{web_data_management_sigmod}, which hinders LLMs' exposure to complex narratives. 
% There have been efforts made in enhancing LLMs' capabilities for long context processing. 
Despite these challenges, significant strides have been made toward enhancing LLMs’ capabilities for long context processing. 

% model architecture
\textbf{Architecture-Based Strategies.} \quad Numerous studies explored the variants of Transformer architecture by modifying its attention mechanism, which includes introducing recurrence~\cite{dai2019transformer}, transforming attention into less computationally demanding forms~\cite{beltagy2020longformer,zaheer2020big}, and employing low-rank approximations~\cite{wang2020linformer,peng2021random}. 
% LONGLLAMAs
Furthermore, LONGLLAMAs~\cite{tworkowski2024focused} presented the Focused Transformer (FOT) featuring a novel training objective that enhances the (key, value) structure, which facilitates the expansion of context length and enables efficient scaling through k-nearest neighbors lookup.
These approaches achieve more efficient exact attention through the development of an IO-optimized CUDA kernel specifically designed for this purpose.


% data construction
% data 和 model 同等重要
\textbf{Data-Centric Approaches.} \quad The effectiveness of long-context language models relies equally upon the innovative employment of data-centric strategies throughout their training processes. 
% Constructing Long-context Training Data. 
% 痛点：cross document attention in long context
The construction of long-context data involves more than a mere concatenation of short documents, which can lead to cross-document attention within a sequence. 
In these circumstances, formulating high-quality or domain-specific long sequences holds significant research value~\cite{devries2023long}. 
% 举例
% ICLM, SPLICE
ICLM~\cite{shi2023context} and SPLICE~\cite{staniszewski2023structured} combine similar training instances through a sophisticated retrieval process, which emphasizes the critical role of high-quality long-context training data in enhancing the context expansion capabilities of LLMs without necessitating extensive data resources.
Additionally, Krell et al.~\cite{krell2021efficient} deliberate on the challenges associated with the conventional concat-and-chunk approach, proposing an approximate bin-packing algorithm as a potential solution. As an improvement, dataset decomposition~\cite{pouransari2024dataset} and Best-fit Packing~\cite{ding2024fewer} both propose the sequence length aware optimization technique to minimize truncations, thereby facilitating more efficient pretraining on long sequences and achieving scalability relative to the size of dataset.
Moreover, ProLong~\cite{chen2024long} introduces an evaluation framework for assessing the quality of long-context data, further enriching the field's methodological toolkit.
% our work
Nonetheless, these methods have not performed a systematic framework tailored for data construction in long context training.
Our work conceptualizes data management for extended-context training as a multi-objective combinatorial optimization problem, and provide a comprehensive framework for long sequence data organization.


% \subsection{Multi-Objective Combinatorial Optimization (MOCO)}
\subsection{\fontsize{10.5}{11.5}\selectfont Multi-Objective Combinatorial Optimization (MOCO)}

Multi-objective combinatorial optimization (MOCO) problems are characterized by the need to optimize multiple objectives simultaneously, which are often in conflict with one another~\cite{ulungu1994multi}. The complexity of MOCO challenges lies in the fact that improving the outcome of one objective often leads to the deterioration of another, making it necessary to find a balance or trade-off between them.

% MOCO 和 LLM 结合举例
\textbf{MOCO-Augmented LLMs.} \quad Existing works have integrated MOCO problems with relevant concerns in the LLMs field.
Wang et al.~\cite{wang2024interpretable} employed the MOCO approach within the Reinforcement Learning from Human Feedback (RLHF) framework for LLMs, where the reward models aggregate multiple reward objectives with coefficients into a scalar score. 
Akiba et al.~\cite{akiba2024evolutionary} viewed model merging as a MOCO challenge, and introduced an innovative approach that leverages evolutionary algorithms to facilitate the automated development of robust foundation models.
% MOCO 与 data selection 结合
Furthermore, integration of MOCO with data-centric LLMs have been explored for training data selection~\cite{du2023mods,xu2023rethinking,chen2024long}, which applies heuristic techniques to assign weights to different data evaluation metrics and facilitates a phased resolution approach.
% our work
Considering the extensive scale of training dataset, data construction for long context is treated as a MOCO challenge, for which the coarse-to-fine algorithm is identified as a suitable resolution strategy.
